Magnetic excitations in Nd$_{n+1}$Ni$_{n}$O$_{3n+1}$ Ruddlesden-Popper nickelates observed via resonant inelastic x-ray scattering

Magnetic interactions are thought to play a key role in the properties of many unconventional superconductors, including cuprates, iron pnictides, and square-planar nickelates. Superconductivity was also recently observed in the bilayer and trilayer Ruddlesden-Popper nickelates, whose electronic structure is expected to differ from that of cuprates and square-planar nickelates. Here we study how electronic structure and magnetic interactions evolve with the number of layers, $n$, in thin film Ruddlesden-Popper nickelates Nd$_{n+1}$Ni$_{n}$O$_{3n+1}$ with $n=1,\:3$, and 5 using resonant inelastic x-ray scattering (RIXS). The RIXS spectra are consistent with a high-spin $|3d^8 \underline{L} \rangle$ electronic configuration, resembling that of La$_{2-x}$Sr$_x$NiO$_4$ and the parent perovskite, NdNiO$_3$. The magnetic excitations soften to lower energy in the structurally self-doped, higher-$n$ films. Our observations confirm that structural tuning is an effective route for altering electronic properties, such as magnetic superexchange, in this prominent family of materials.

==> latexmkrc <==
# Use pound symbols to comment lines that you do not want to run

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

# main text
#$pdflatex = "latexdiff OLD.tex main.tex  > main-d.tex; pdflatex %O  main-d"

# supp
#$pdflatex = "latexdiff supp_old.tex supp.tex  > main-d.tex; pdflatex %O  main-d"

